Monitoring Hyperproperties

Hyperproperties, such as non-interference and observational determinism, relate multiple system executions to each other. They are not expressible in standard temporal logics, like LTL, CTL, and CTL*, and thus cannot be monitored with standard runtime verification techniques. HyperLTL extends linear-time temporal logic (LTL) with explicit quantification over traces in order to express Hyperproperties. We investigate the runtime verification problem of HyperLTL formulas for three different input models: (1) The parallel model, where a fixed number of system executions is processed in parallel. (2) The unbounded sequential model, where system executions are processed sequentially, one execution at a time. In this model, the number of incoming executions may grow forever. (3) The bounded sequential model where the traces are processed sequentially and the number of incoming executions is bounded. We show that deciding monitorability of HyperLTL formulas is PSPACE-complete for input models (1) and (3). Deciding monitorability is PSPACE-complete for alternation-free HyperLTL formulas in input model (2). For every input model, we provide practical monitoring algorithms. We also present various optimization techniques. By recognizing properties of specifications such as reflexivity, symmetry, and transitivity, we reduce the number of comparisons between traces. For the sequential models, we present a technique that minimized the number of traces that need to be stored. Finally, we provide an optimization that succinctly represents the stored traces by sharing common prefixes. We evaluate our optimizations, showing that this leads to much more scalable monitoring, in particular, significantly lower memory consumption.

==> alternations.tex <==
\section{Monitoring Alternating $\hyperltl$ Formulas}
\label{sec:alternation}

With the classic definition of monitorability (cf.~Section~\ref{sec:monitorability}), hardly any alternating $\hyperltl$ formula is monitorable as their satisfaction cannot be characterized by a finite trace set, even for safety properties.
Consider, for example, the formula $\varphi = \forall \pi \ldot \exists \pi' \ldot \G (a_\pi \rightarrow b_{\pi'})$.
Assume a finite set of traces $T$ does not violate the formula.
Then, one can construct a new trace $t$ where $a \in t[i]$ and $b \notin t[i]$ for some position $i$, and for all traces $t' \in T$ it holds that $b \notin t'[i]$.
Thus, the new trace set violates $\varphi$.
Likewise, if there is a finite set of traces that violates $\varphi$, a sufficiently long trace containing only $b$'s stops the violation.

If we fix a set of traces, we can check the satisfaction of an alternating $\hyperltl$ formula with a modification of the offline monitoring algorithm presented earlier.
This way, we can verify alternating hyperproperties after the execution of a system based on recorded traces.
In our conference management system example, the property \emph{``There was a submission for every paper that is visible for a program committee member.''} is a hyperproperty that utilizes alternation and can be formalized as the $\forall\exists\hyperltl$ formula
\begin{equation}  \label{eq:conference-management-alternating}
  \forall \pi \ldot \exists \pi' \ldot pc_{\pi'} \wedge (\neg pc_\pi \rightarrow \X\G (s_\pi \rightarrow \X v_{\pi'})) \enspace .
\end{equation}
In the following, we present an extension to our offline algorithm for monitoring $\forall\exists\hyperltl$ and $\exists\forall\hyperltl$ formulas.
Further, we show that the trace storage minimization technique is also applicable for alternating $\hyperltl$ formulas, allowing to determine at runtime whether a trace needs to be stored or not.

%A basic solution for this problem is to consider \emph{offline} monitoring, where traces are stored subsequently and evaluated after the system terminates.
%In the worst case, however, we have to store every trace in order to soundly check whether or not this trace set violates the hyperproperty under consideration.
%In this section, we show how to use the trace analysis technique presented above for equipping a trace gathering procedure with an online method that minimizes, with respect to a hyperproperty, the trace set that needs to be stored.

%\subsection{Offline Monitoring}
We considered offline monitoring of universally quantified $\forall^n\hyperltl$ in Section~\ref{sec:monitoringhyperltl} by checking whether $\monitor_{\varphi}$ accepts $N$ for every $N \in T^n$, given a trace set $T$ and a $\hyperltl$ formula $\varphi$.
In contrast, an offline monitor for a $\forall^n \exists^m \hyperltl$ and $\exists^m \forall^n \hyperltl$ formula has to perform the checks
\begin{align*}
  &\bigwedge_{N \in T^n} \bigvee_{M \in T^m} \text{check if } \monitor_{\varphi} \text{ accepts } N \times M \enspace\text{, and}\\
  &\bigvee_{M \in T^m} \bigwedge_{N \in T^n} \text{check if } \monitor_{\varphi} \text{ accepts } M \times N \enspace \text{, respectively.} 
\end{align*}

We give a characterization of the trace dominance introduced in the last section for $\hyperltl$ formulas with one alternation.
These characterizations can be checked similarly to the algorithm depicted in Fig.~\ref{alg_minimization}.
\begin{theorem} \label{thm:forall-exists-dominance}
  Given a $\hyperltl$ formula $\forall \pi \ldot \exists \pi' \ldot \psi$ two traces $t,t' \in \traces$, the following holds: $t$ dominates $t'$ if and only if
  \begin{equation*}
    \lang(\monitor_\varphi[t/\pi]) \subseteq \lang(\monitor_\varphi[t'/\pi])
    \text{ and }
    \lang(\monitor_\varphi[t'/\pi']) \subseteq \lang(\monitor_\varphi[t/\pi']) \enspace.
  \end{equation*}
\end{theorem}
\begin{proof}
  The $\Rightarrow$ direction is the same as in proofs of Theorem~\ref{dominating} and Lemma~\ref{thm:exists-2-dominance}.
  
  For the other direction, assume that that (a) $\lang(\monitor_\varphi[t/\pi]) \subseteq \lang(\monitor_\varphi[t'/\pi])$ and (b) $\lang(\monitor_\varphi[t'/\pi']) \subseteq \lang(\monitor_\varphi[t/\pi'])$.
  Let $T'$ be arbitrary such that $\set{t} \subseteq T'$.
  We distinguish two cases:
  \begin{itemize}
    \item
      Case $T' \in \lang(\varphi)$, then for all $t_1 \in T'$ there is a $t_2 \in T'$ such that $\pathassignfin = \set{\pi \mapsto t_1, \pi' \mapsto t_2} \models_\emptyset \psi$.
      Especially, for $t$, there is a corresponding trace $t^*$ such that $\set{\pi \mapsto t, \pi' \mapsto t^*} \models_\emptyset \psi$, thus $t^* \in \lang(\monitor_\varphi[t/\pi])$.
      From (a) it follows that $t^* \in \lang(\monitor_\varphi[t'/\pi])$.
      Hence, $\set{\pi \mapsto t', \pi' \mapsto t^*} \models_\emptyset \psi$ and thereby $T' \cup \set{t'} \in \lang(\varphi)$.
    \item
      Case $T' \cup \set{t'} \in \lang(\varphi)$, then for all $t_1 \in T' \cup \set{t'}$ there is a $t_2 \in T' \cup \set{t'}$ such that $\set{\pi \mapsto t_1, \pi' \mapsto t_2} \models_\emptyset \psi$.
      Assume for the sake of contradiction there is a $t_1 \in T'$ such that there is no $t_2 \in T'$ with $\set{\pi \mapsto t_1, \pi' \mapsto t_2} \models_\emptyset \psi$.
      It follows that $\set{\pi \mapsto t_1, \pi' \mapsto t'} \models_\emptyset \psi$, i.e., $t_1 \in \lang(\monitor_\varphi[t'/\pi'])$.
      From (b) it follows that $t_1 \in \lang(\monitor_\varphi[t/\pi'])$, leading to the contradiction that $\set{\pi \mapsto t_1, \pi' \mapsto t} \models_\emptyset \psi$ and $t \in T'$.
      Hence, $T' \in \lang(\varphi)$.
  \end{itemize}
\end{proof}
\begin{corollary}
  Given a $\hyperltl$ formula $\exists \pi \ldot \forall \pi' \ldot \psi$ two traces $t,t' \in \traces$, the following holds: $t$ dominates $t'$ if and only if
  \begin{equation*}
    \lang(\monitor_\varphi[t'/\pi]) \subseteq \lang(\monitor_\varphi[t/\pi])
    \text{ and }
    \lang(\monitor_\varphi[t/\pi']) \subseteq \lang(\monitor_\varphi[t'/\pi']) \enspace.
  \end{equation*}
\end{corollary}

\begin{example}
  We show the effect of the dominance characterization on two example formulas.
	Consider the $\hyperltl$ formula $\forall \pi \ldot \exists \pi' \ldot \G (a_\pi \rightarrow b_{\pi'})$ and the traces $\set{b} \emptyset$, $\set{b}\set{b}$, $\set{a} \emptyset$, and $\set{a}\set{a}$.
	Trace $\set{a}\set{a}$ dominates trace $\set{a}\emptyset$ as instantiating $\pi$ requires two consecutive $b$'s for $\pi'$ where $\set{a}\emptyset$ only requires a $b$ at the first position (both traces do not contain $b$'s, so instantiating $\pi'$ leads to the same language).
	Similarly, one can verify that $\set{b}\set{b}$ dominates trace $\set{b}\emptyset$.
	
	Consider alternatively the formula $\exists \pi \ldot \forall \pi' \ldot \G (a_\pi \rightarrow b_{\pi'})$.
	In this case, $\set{a}\emptyset$ dominates $\set{a}\set{a}$ and $\set{b}\emptyset$ dominates $\set{b}\set{b}$.
\end{example}
For our conference management example formula given in Equation~\ref{eq:conference-management-alternating}, a trace $\set{pc}\emptyset\set{v}$ dominates $\set{pc}\emptyset\emptyset$ and $\emptyset\set{s}\emptyset$ dominates $\emptyset\emptyset\emptyset$, but $\emptyset\set{s}\emptyset$ and $\set{pc}\emptyset\set{v}$ are incomparable with respect to the dominance relation.

%\subsection{Trace Storage Minimization for Alternating $\hyperltl$ Formulas}


==> different_input_models.tex <==
\section{Different Input Models}

In general, we distinguish between two different input models. In the first model, traces are processed sequentially, i.e., given a set of traces $T$ and a fresh trace $t$, the monitoring algorithm has to decide whether $T \cup t$ satisfies or violates a given $\hyperltl$ formula before processing another fresh traces $t'$.
In the second model, traces of a fixed trace set $T$ are processed in parallel. Note that in the second model the trace set $T$ is of fixed size and, in contrast to the first input model, not allowed to grow. Figure~\ref{} sketches the differences between both input models. This distinction has major effects on the monitorability of $\hyperltl$ formulas.
In the first subsection, we will consider monitorability of $\hyperltl$ formulas in the parallel model, before considering the sequential model.

\subsection{Monitorability in the Parallel Model}
.

\subsection{Monitorability in the Sequential Model}
We present a method to decide whether an alternation-free $\hyperltl$ formula is monitorable.

%\begin{remark}
%  Defining $\good(H)$ (respectively $\bad(H)$) only over finite subsets of $\Sigma^*$ is no restriction for properties given in $\hyperltl$ (cf.~Lemma~\ref{thm:forall-good-empty}).
%\end{remark}

\begin{lemma}\label{thm:forall-good-empty}
  Given a $\hyperltl$ formula $\varphi = \forall \pi_1 \dots \forall \pi_k \ldot \psi$, where $\psi$ is an $\ltl$ formula.
  It holds that $\good(\lang(\varphi)) = \emptyset$ unless $\psi \equiv \true$.
\end{lemma}
\begin{proof}
	If $\psi \equiv \true$ then $\lang(\varphi) = \powerset(\Sigma^\omega)$ and $\good(\lang(\varphi)) = \powerset^*(\Sigma^*)$.
	Assume for contradiction that $\psi \not\equiv \true$ and $\good(\lang(\varphi)) \neq \emptyset$, i.e., there is a finite set $U \subseteq \Sigma^*$ that is a good prefix set of $\varphi$.
	Since $\psi \neq \true$, there is at least one infinite trace $\sigma$ with $\sigma \nmodels \psi$.
	We translate this trace to a set of infinite traces $W$ where $W \nmodels \varphi$ using Lemma~\ref{thm:hyperltl-body-to-ltl}.
	Further, for all $V \in \powerset(\Sigma^*)$ with $U \pref V$, it holds that $W \subseteq V$, hence, $V \notin \lang(\varphi)$ violating the assumption that $U \in \good(\lang(\varphi))$.
	\qed
\end{proof}



\begin{theorem} \label{thm:monitorability-forall}
  Given a $\hyperltl$ formula $\varphi = \forall \pi_1 \dots \forall \pi_k \ldot \psi$, where $\psi \not\equiv \true$ is an $\ltl$ formula.
  $\varphi$ is monitorable if, and only if, $\forall u \in \Sigma_\pathvars^* \ldot \exists v \in \Sigma_\pathvars^* \ldot uv \in \bad(\lang(\psi))$.
\end{theorem}
\begin{proof}%\hfill
%\begin{itemize}
%  \item[$\Leftarrow$]
    Assume $\forall u \in \Sigma_\pathvars^* \ldot \exists v \in \Sigma_\pathvars^* \ldot uv \in \bad(\lang(\psi))$ holds.
    Given an arbitrary prefix $U \in \powerset^*(\Sigma^*)$.
    Pick an arbitrary mapping from $U$ to $\Sigma^*_\pathvars$ and call it $u'$.
    By assumption, there is a $v' \in \Sigma^*_\pathvars$ such that $u'v' \in \bad(\lang(\psi))$.
    We use this $v'$ to extend the corresponding traces in $U$ resulting in $V \in \powerset^*(\Sigma^*)$.
    %\tbchecked{It seems that one has to allow ``splitting'' of prefix paths, consider for example a model consisting of a single trace, but two path variables: bot path variables map to the same path, but the $\ltl$ formula can consider different extensions because the atomic propositions are different.}
    It follows that for all $W \in \powerset(\Sigma^\omega)$ with $V \pref W$, $W \nmodels \varphi$, hence, $V \in \bad(\lang(\varphi))$.
    
  
%  \item[$\Rightarrow$]
    %\tbchecked{This direction does not hold if $\psi \equiv \true$ as $\varphi$ is monitorable, but $\bad(\lang(\true)) = \emptyset$. Is $\psi \equiv \true$ the only additional restriction to satisfy the claim?}
    Assume $\varphi$ is monitorable, thus, $\forall U \in \powerset^*(\Sigma^*) \ldot \exists V \in \powerset^*(\Sigma^*) \ldot U \pref V \implies V \in \good(\lang(\varphi)) \lor V \in \bad(\lang(\varphi))$.
    As the set of good prefixes $\good(\lang(\varphi))$ is empty by Lemma~\ref{thm:forall-good-empty} we can simplify the formula to $\forall U \in \powerset^*(\Sigma^*) \ldot \exists V \in \powerset^*(\Sigma^*) \ldot U \pref V \implies V \in \bad(\lang(\varphi))$.
%    
    Given an arbitrary $u \in \Sigma_\pathvars^*$, we translate it into the (canonical) $U'$ and get a $V'$ satisfying the conditions above.
    Let $v' \in \Sigma_\pathvars^*$ be the finite trace constructed from the extensions of $u$ in $V'$ (not canonical, but all are bad prefixes since $V' \in \bad(\lang(\varphi))$).
    By assumption, $u'v' \in \bad(\lang(\psi))$.
    \qed
%\end{itemize}
\end{proof}

\begin{corollary}
  Given a $\hyperltl$ formula $\varphi = \exists \pi_1 \dots \exists \pi_k. \psi$, where $\psi$ is an $\ltl$ formula.
  $\varphi$ is monitorable if, and only if, $\forall u \in \Sigma_\pathvars^* \ldot \exists v \in \Sigma_\pathvars^* \ldot uv \in \good(\lang(\psi))$.
\end{corollary}


\begin{theorem}
  Given an alternation-free $\hyperltl$ formula $\varphi$.
  Deciding whether $\varphi$ is monitorable is $\pspace$-complete.
\end{theorem}
\begin{proof}
  We consider the case that $\varphi = \forall \pi_1 \dots \forall \pi_2 \ldot \psi$, the case for existentially quantified formulas is dual.
  We apply the characterization from Theorem~\ref{thm:monitorability-forall}.
  First, we have to check validity of $\psi$ which can be done in polynomial space~\cite{conf/stoc/SistlaC82}.
  Next, we have to determine whether $\forall u \in \Sigma_\pathvars^* \ldot \exists v \in \Sigma_\pathvars^* \ldot uv \in \bad(\lang(\psi))$.
  We use a slight modification of the $\pspace$ algorithm given by Bauer~\cite{journals/corr/abs-1006-3638}.
  Hardness follows as the problem is already $\pspace$-hard for $\ltl$.
  \qed
\end{proof}


==> monitorability.tex <==
\section{Monitorability of HyperLTL}
\label{prelim}
Let $\ap$ be a finite set of atomic propositions and let $\Sigma = 2^\ap$ be the corresponding finite \emph{alphabet}.
A finite (infinite) trace is a finite (infinite) sequence over $\Sigma$.
%
We denote the concatenation of a finite trace $u \in \Sigma^*$ and a finite or infinite trace $v \in \Sigma^* \cup \Sigma^\omega$ by $uv$ and write $u \pref v$ if $u$ is a prefix of $v$.
Further, we lift the prefix operator to sets of traces, i.e., $U \pref V \coloneqq \forall u \in U \ldot \exists v \in V \ldot u \pref v$ for $U \subseteq \Sigma^*$ and $V \subseteq \Sigma^* \cup \Sigma^\omega$.
We denote the powerset of a set $A$ by $\powerset(A)$ and define $\powerset^*(A)$ to be the set of all finite subsets of $A$.


\subsection{HyperLTL.}

$\hyperltl$~\cite{conf/post/ClarksonFKMRS14} is a temporal logic for specifying hyperproperties.
It extends $\ltl$~\cite{conf/focs/Pnueli77} by quantification over trace variables $\pi$ and a method to link atomic propositions to specific traces.
The set of trace variables is $\pathvars$.
Formulas in $\hyperltl$ are given by the grammar
\begin{align*}
  \varphi &{}\Coloneqq \forall\pi\ldot\varphi \mid \exists\pi\ldot\varphi \mid \psi \enspace, \text{ and}\\
  \psi &{}\Coloneqq a_\pi \mid \neg\psi \mid \psi\lor\psi \mid \X\psi \mid \psi\U\psi \enspace,
\end{align*}
where $a \in \ap$ and $\pi \in \pathvars$.
We call a $\hyperltl$ formula an $\ltl$ formula if it is quantifier free.
%
The semantics is given by the satisfaction relation $\models_P$ over a set of traces $T \subseteq \Sigma^\omega$.
We define an assignment $\pathassign : \pathvars \to \Sigma^\omega$ that maps trace variables to traces. $\pathassign[i,\infty]$ denotes the trace assignment that is equal to $\pathassign(\pi)[i,\infty]$ for all $\pi$.
\begin{equation*}
\begin{array}{ll}
  \pathassign \models_T a_\pi         \qquad \qquad & \text{if } a \in \pathassign(\pi)[0] \\
  \pathassign \models_T \neg \varphi              & \text{if } \pathassign \nmodels_T \varphi \\
  \pathassign \models_T \varphi \lor \psi         & \text{if } \pathassign \models_T \varphi \text{ or } \pathassign \models_T \psi \\
  \pathassign \models_T \X \varphi                & \text{if } \pathassign[1,\infty] \models_T \varphi \\
  \pathassign \models_T \varphi\U\psi             & \text{if } \exists i \geq 0 \ldot \pathassign[i,\infty] \models_T \psi \land \forall 0 \leq j < i \ldot \pathassign[j,\infty] \models_T \varphi \\
  \pathassign \models_T \exists \pi \ldot \varphi & \text{if there is some } t \in T \text{ such that } \pathassign[\pi \mapsto t] \models_T \varphi
\end{array}
\end{equation*}
%
We write $T \models \varphi$ for $\set{} \models_T \varphi$ where $\set{}$ denotes the empty assignment.
The language of a $\hyperltl$ formula $\varphi$, denoted by $\lang(\varphi)$, is the set $\set{ T \subseteq \Sigma^\omega \mid T \models \varphi }$.
%
Let $\varphi$ be a $\hyperltl$ formula with trace variables $\pathvars = \set{\pi_1,\dots,\pi_k}$ over alphabet $\Sigma$.
We define $\Sigma_\pathvars$ to be the alphabet where $p_\pi$ is interpreted as an atomic proposition for every $p \in \ap$ and $\pi \in \pathvars$.
We denote by $\models_\ltl$ the $\ltl$ satisfaction relation over $\Sigma_\pathvars$.
We define the $\pi$-projection, denoted by $\#_\pi(s)$, for a given $s \subseteq \Sigma_\pathvars$ and $\pi \in \pathvars$, as the set of all $p_\pi \in s$.
  
\begin{lemma} \label{thm:hyperltl-body-to-ltl}
  Let $\psi$ be an $\ltl$ formula over trace variables $\pathvars$.
  There is a trace assignment $A$ such that $A \models_\emptyset \psi$ if, and only if, $\psi$ is satisfiable under $\ltl$ semantics over atomic propositions $\Sigma_\pathvars$.
  The models can be translated effectively.
\end{lemma}
\begin{proof}
	Assume that there is a trace assignment $A$ over trace variables $\pathvars$ such that $A \models_\emptyset \psi$.
	We define $w \subseteq \Sigma_\pathvars^\omega$ such that $x_\pi \in w[i]$ if, and only if, $x \in A(\pi)[i]$ for all $i \geq 0$, $x \in \ap$, and $\pi \in \pathvars$.
	An induction over $\psi$ shows that $w \models_\ltl \psi$.
	
	Assume $\psi$ is satisfiable for $\models_\ltl$, i.e., there exists a $w \subseteq \Sigma^\omega_\pathvars$, such that $w \models_\ltl \psi$.
	We construct an assignment $A$ in the following manner: Let $\pi \in \pathvars$ be arbitrary.
	We map $\pi$ to the trace $t$ obtained by projecting the corresponding $p_\pi \in \Sigma_\pathvars$, i.e., $\forall i \geq 0 \ldot t[i] = \#_\pi(w[i])$.
	\qed
\end{proof}

\subsection{Finite Trace Semantics of HyperLTL.}
We define a finite trace semantics for $\hyperltl$ based on the finite trace semantics of LTL~\cite{books/daglib/0080029}.
In the following, when using $\lang(\varphi)$ we refer to the finite trace semantics of a $\hyperltl$ formula $\varphi$.
Let $t$ be a finite trace, $\epsilon$ denotes the empty trace, and $|t|$ denotes the length of a trace. Since we are in a finite trace setting, $t[i,\ldots]$ denotes the subsequence from position $i$ to position $|t|-1$.
Let $\pathassignfin : \pathvars \rightarrow \Sigma^*$ be a partial function mapping trace variables to finite traces. We define $\epsilon[0]$ as the empty set.
$\pathassignfin[i, \ldots]$ denotes the trace assignment that is equal to $\pathassignfin(\pi)[i,\ldots]$ for all $\pi$. We define a subsequence of $t$ as follows.
\[
t[i,j] = \begin{cases}
\epsilon & \text{if } i \geq |t|\\
t[i,\textit{min}(j,|t|-1)], & \text{otherwise}
\end{cases}
\]
\begin{equation*}
\begin{array}{ll}
\pathassignfin \models_T a_\pi         \qquad \qquad & \text{if } a \in \pathassignfin(\pi)[0] \\
\pathassignfin \models_T \neg \varphi              & \text{if } \pathassignfin \nmodels_T \varphi \\
\pathassignfin \models_T \varphi \lor \psi         & \text{if } \pathassignfin \models_T \varphi \text{ or } \pathassignfin \models_T \psi \\
\pathassignfin \models_T \X \varphi                & \text{if } \pathassignfin[1,\ldots] \models_T \varphi \\
%F \models_P \tilde{\X} \varphi                & \text{if } F[1,\ldots] \models_P \varphi \\
\pathassignfin \models_T \varphi\U\psi             & \text{if } \exists i \geq 0 \ldot \pathassignfin[i,\ldots] \models_T \psi \land \forall 0 \leq j < i \ldot \pathassignfin[j,\ldots] \models_T \varphi \\
\pathassignfin \models_T \exists \pi \ldot \varphi & \text{if there is some } t \in T \text{ such that } \pathassignfin[\pi \mapsto t] \models_T \varphi
\end{array}
\end{equation*}

\subsection{Monitorability.} \label{sec:monitorability}

%In the remainder of this section, we recap the notion of monitorability for hyperproperties and show that deciding whether a $\hyperltl$ formula is monitorable is $\pspace$-complete, i.e., no harder than the corresponding problem for $\ltl$.
%This result extends earlier characterizations based on restricted syntactic fragments of $\hyperltl$~\cite{conf/csfw/AgrawalB16}.

For trace languages, monitorability is the property whether language containment can be decided by finite prefixes~\cite{conf/fm/PnueliZ06}.
Given a trace language $L \subseteq \Sigma^\omega$, the set of \emph{good} and \emph{bad} prefixes is $\good(L) \coloneqq \set{u \in \Sigma^* \mid \forall v \in \Sigma^\omega \ldot uv \in L}$ and $\bad(L) \coloneqq \set{u \in \Sigma^* \mid \forall v \in \Sigma^\omega \ldot uv \notin L}$, respectively.
$L$ is \emph{monitorable} if $\forall u \in \Sigma^* \ldot \exists v \in \Sigma^* \ldot uv \in \good(L) \lor uv \in \bad(L)$.
%
The decision problem, i.e., given an $\ltl$ formula $\varphi$, decide whether $\varphi$ is monitorable, is $\pspace$-complete~\cite{journals/corr/abs-1006-3638}.

A \emph{hyperproperty} $H$ is a set of trace properties, i.e., $H \subseteq \powerset(\Sigma^\omega)$.
Analogous to the previous definition, we define monitorability for hyperproperties.
Given $H \subseteq \powerset(\Sigma^\omega)$.
The set of \emph{good} and \emph{bad prefix traces} is $\good(H) \coloneqq \set{U \in \powerset^*(\Sigma^*) \mid \forall V \in \powerset(\Sigma^\omega) \ldot U \pref V \implies V \in H}$ and $\bad(H) \coloneqq \set{U \in \powerset^*(\Sigma^*) \mid \forall V \in \powerset(\Sigma^\omega) \ldot U \pref V \implies V \notin H}$, respectively.
$H$ is \emph{monitorable} if
\begin{equation*}
	\forall U \in \powerset^*(\Sigma^*) \ldot \exists V \in \powerset^*(\Sigma^*) \ldot U \pref V \implies V \in \good(H) \lor V \in \bad(H) \enspace.
\end{equation*}


==> monitoring-hyperltl.tex <==
\section{Monitoring HyperLTL}
\label{sec:monitoringhyperltl}
There are many obstacles to overcome in monitoring hyperproperties (see~\cite{conf/rv/BonakdarpourF16} for an overview of the challenges), such that classic monitoring approaches of trace properties need to be carefully adjusted.
In this section, we define a finite trace semantics for $\hyperltl$ and present our automata-based monitoring approach.


\subsection{Finite Trace Semantics.}
We define a finite trace semantics for $\hyperltl$ based on the finite trace semantics of LTL~\cite{books/daglib/0080029}.
In the following, when using $\lang(\varphi)$ we refer to the finite trace semantics of a $\hyperltl$ formula $\varphi$.
Let $t$ be a finite trace, $\epsilon$ denotes the empty trace, and $|t|$ denotes the length of a trace. Since we are in a finite trace setting, $t[i,\ldots]$ denotes the subsequence from position $i$ to position $|t|-1$.
Let $\pathassignfin : \pathvars \rightarrow \Sigma^*$ be a partial function mapping trace variables to finite traces. We define $\epsilon[0]$ as the empty set.
$\pathassignfin[i, \ldots]$ denotes the trace assignment that is equal to $\pathassignfin(\pi)[i,\ldots]$ for all $\pi$. We define a subsequence of $t$ as follows.
\[
t[i,j] = \begin{cases}
\epsilon & \text{if } i \geq |t|\\
t[i,\textit{min}(j,|t|-1)], & \text{otherwise}
\end{cases}
\]
\begin{equation*}
\begin{array}{ll}
\pathassignfin \models_T a_\pi         \qquad \qquad & \text{if } a \in \pathassignfin(\pi)[0] \\
\pathassignfin \models_T \neg \varphi              & \text{if } \pathassignfin \nmodels_T \varphi \\
\pathassignfin \models_T \varphi \lor \psi         & \text{if } \pathassignfin \models_T \varphi \text{ or } \pathassignfin \models_T \psi \\
\pathassignfin \models_T \X \varphi                & \text{if } \pathassignfin[1,\ldots] \models_T \varphi \\
%F \models_P \tilde{\X} \varphi                & \text{if } F[1,\ldots] \models_P \varphi \\
\pathassignfin \models_T \varphi\U\psi             & \text{if } \exists i \geq 0 \ldot \pathassignfin[i,\ldots] \models_T \psi \land \forall 0 \leq j < i \ldot \pathassignfin[j,\ldots] \models_T \varphi \\
\pathassignfin \models_T \exists \pi \ldot \varphi & \text{if there is some } t \in T \text{ such that } \pathassignfin[\pi \mapsto t] \models_T \varphi
\end{array}
\end{equation*}


\subsection{Monitoring Algorithm.}
In this subsection, we describe our automata-based monitoring algorithm for $\hyperltl$.
We employ standard techniques for building LTL monitoring automata and use this to instantiate this monitor by the traces as specified by the $\hyperltl$ formula.

Let $\ap$ be a set of atomic propositions and $\pathvars = \{\pi_1, \ldots, \pi_n\}$ a set of trace variables. 
A deterministic monitor template $\monitor = (\Sigma, Q, \delta, q_0)$ is a four tuple of
a finite alphabet $\Sigma = 2^{\ap \times \pathvars}$,
a non-empty set of states $Q$,
a partial transition function $\delta: Q \times \Sigma \rightarrow Q$,
and a designated initial state $q_0 \in Q$.
The automata runs in parallel over traces $(2^\ap)^*$, thus we define a run with respect to a $n$-ary tuple $N \in ((2^\ap)^*)^n$ of finite traces.
A run of $N$ is a sequence of states $q_0 q_1 \cdots q_m \in Q^*$, where $m$ is the length of the smallest trace in $N$, starting in the initial state $q_0$ such that for all $i$ with $0 \leq i < m$ it holds that 
\begin{equation*}
  \delta\left(q_i, \bigcup_{j=1}^n \bigcup_{a \in N(j)(i)} \set{(a,\pi_j)} \right) = q_{i+1} \enspace.
\end{equation*}
A tuple $N$ is accepted, if there is a run on $\monitor$.
For LTL, such a deterministic monitor can be constructed in doubly-exponential time in the size of the formula~\cite{conf/cav/dAmorimR05,journals/fmsd/TabakovRV12}.
%To simplify notation, we identify a path assignment $\pathassign$ over path variables $\pathvars = \set{\pi_1,\dots,\pi_n}$ by a $n$-ary tuple.

\begin{example}
  We consider again the conference management example from the introduction.
  We distinguish two types of traces, \emph{author traces} and \emph{program committee member traces}, where the latter starts with proposition $pc$.
  Based on this traces, we want to verify that no paper submission is lost, i.e., that every submission (proposition $s$) is visible (proposition $v$) to every program committee member in the following step.
  When comparing two PC traces, we require that they agree on proposition $v$. The monitor template for the following $\hyperltl$ formalization is depicted in Fig.~\ref{fig:monitor-template}.
  \begin{equation} \label{eq:conference-management-visibility}
    \forall \pi. \forall \pi' \ldot \big((\neg pc_\pi \wedge pc_{\pi'}) \rightarrow \X\G (s_\pi \rightarrow \X v_{\pi'})\big) \wedge \big((pc_{\pi} \wedge pc_{\pi'}) \rightarrow \X\G (v_\pi \leftrightarrow v_\pi')\big)
  \end{equation}
\end{example}
\begin{figure}[t]
  \centering
  \input{./tikz/monitor_conference_example}
  \caption{Visualization of a monitor template corresponding to formula given in Equation~\ref{eq:conference-management-visibility}. We use a symbolic representation of the transition function $\delta$.}
  \label{fig:monitor-template}
  \vspace{-10pt}
\end{figure}

The offline and online algorithms for monitoring $\hyperltl$ formulas are presented in Fig.~\ref{fig:offline-online-algorithm}.
The \emph{offline} algorithm takes a $\hyperltl$ formula $\varphi$ and a set of traces $T$ as input.
After building the deterministic monitoring automaton $\monitor_\varphi$, it checks every $n$-ary tuple $N \in T^n$.
If some trace tuple $N$ is not accepted by $\monitor_\varphi$, then this path assignment violates the formula $\varphi$.
%
The \emph{online} algorithm is similar, but proceeds with the pace of the incoming stream, which has an indicator when a new trace starts.
We have a variable $S$ that maps tuples of traces to states of the deterministic monitor.
Whenever a trace progresses, we update the states in $S$ according to the transition function $\delta$.
If on this progress, there is a violation, we return the corresponding tuple of traces as a witness.
When a new trace $t$ starts, only new tuples are considered for $S$, that are tuples $N \in (T \cup \set{t})^n$ containing the new trace $t$, i.e., $N \notin T^n$.

%We use the monitor generation from Spot, which is described in~\cite{}\todo{cite beide papiere aus email, Formal Konstruktion aufschreiben?}, based on a BDD representation of the alphabet. An \emph{instance} of a monitor template $\monitor_{i_1,\ldots,i_n} = (\Sigma', Q', \delta', q_0')$ is constructed as follows:
%\begin{align*}
%&\Sigma' \coloneqq \left(2^{\ap}\right)^{n}\\
%&Q' \coloneqq Q\\
%&\delta'(q,(l_{i_1}, \ldots, l_{i_n})) \coloneqq \delta(q, \bigcup_{j=1}^n l_{i_j} \times \{\pi_j\})\\
%&q'_0 \coloneqq q_0,
%\end{align*}
%We say a monitor template accepts trace set $T$ if every possible initialization is accepted by the corresponding automatons, denoted by $T \subseteq M$.\todo{!}

%\begin{example}
%\begin{figure}
%  \centering
%  \input{./tikz/example_monitor}
%  \caption{Monitor for $\ltl$ formula $\G (a_\pi \leftrightarrow a_{\pi'})$.}
%  \label{fig:example_monitor_template}
%\end{figure}
%Consider the $\hyperltl$ formula $\forall \pi \forall \pi' \ldot \G (a_\pi \leftrightarrow a_{\pi'})$.
%We build the monitor template, depicted in Fig.~\ref{fig:example_monitor_template}, from the $\ltl$ formula.
%Given a set of input traces $\Pi = \set{\pi_1,\dots,\pi_n}$, for every pair $(\pi_i,\pi_j) \in \Pi \times \Pi$, we instantiate a new monitor $\monitor_{i,j}$ from the template.
%Then, these monitors are progressing according to the template.
%
%For example,~\todo{eher tau statt pi?} given three input traces $\pi_1, \pi_2, \pi_3$, we instanciate $8$ monitor automata $\monitor_{1,1}$, $ \monitor_{1,2}$, $\monitor_{1,3}$, $\monitor_{2,1}$, $\monitor_{2,2}$, $\monitor_{2,3}$, $\monitor_{3,1}$, $\monitor_{3,2}$, and $\monitor_{3,3}$.
%\end{example}
%In general, when we have $n$ path quantifier and $m$ input paths, we need $m^n$ many monitor automata.
%\todo{What about input paths with different lengths?}\\
%Currently our algorithm only steps through the monitor instances whose corresponding input paths have not yet ended, i.e., as soon as a input path ends we assume to stay in a valid state for those monitor automata. 
%\subsection{Sequential Monitoring}
%Sequential monitoring describes the variant of monitoring where the paths are given one after another.
\begin{figure}[t]
\hspace{-10pt}
\centering
\scalebox{.9}{
\begin{minipage}{0.46\textwidth}
\begin{algorithm}[H]
	\SetKwInOut{Input}{input}
	\SetKwInOut{Output}{output}
	\SetAlgoLined
	%\KwResult{Write here the result }
	\Input{$\forall^n$ HyperLTL formula $\varphi$\\
	       set of traces $T$}
	\Output{satisfied or $n$-ary tuple\\witnessing violation}
	\BlankLine
	$\monitor_\varphi =$ \texttt{build\_template($\varphi$)}\;
	\BlankLine
		\For{each tuple $N \in T^n$}{
		\eIf{$\monitor_\varphi$ accepts $N$}{
			proceed\;
		}{
		    \Return $N$\;
		}
	}
	\Return satisfied\;
	\BlankLine
	\caption{Offline Algorithm.}
\end{algorithm}
\end{minipage}%
\begin{minipage}{0.65\textwidth}
\begin{algorithm}[H]
	\SetKwInOut{Input}{input}
	\SetKwInOut{Output}{output}
	\SetAlgoLined
	%\KwResult{Write here the result }
	\Input{$\forall^n$ HyperLTL formula $\varphi$}
	\Output{satisfied or $n$-ary tuple\\witnessing violation}
	\BlankLine
	$\monitor_\varphi = (\Sigma, Q, \delta, q_0) =$ \texttt{build\_template($\varphi$)}\;
	$S: T^n \rightarrow Q$\;
	$T \coloneqq \emptyset$\;
	$t \coloneqq \epsilon$\;
	\BlankLine
	\While{$p \leftarrow$ new element}{
		\eIf{$p$ is new trace}{
			$T \cup \{t\}$\;
			$t \coloneqq \epsilon$\;
			$S \coloneqq \set{q_0 \mid \text{for new $n$-tuple}}$\;
		}{
			$t \coloneqq t~p$\;
			progress every state in $S$ according to $\delta$\;
			\If{violation}{
				\Return witnessing tuple\;
			}
		}
	}
	\Return satisfied\;
	\BlankLine
	\caption{Online Algorithm.}
\end{algorithm}
\end{minipage}
}
\caption{Evaluation algorithms for monitoring $\forall^n$ HyperLTL formulas.}
\label{fig:offline-online-algorithm}
\vspace{-10pt}
\end{figure}

%\begin{definition}{Monitoring Algorithm}
%\begin{enumerate}
%    \item build monitor template from LTL part of the formula via Spot
%    \item check if monitor represents FALSE $\Rightarrow$ throw error
%    \item for each new path repeat following steps 4.-9.
%    \item instanciate new monitors, i.e., not yet seen path combinations only
%    \item for each label in new path repeat following steps 6.-9.
%    \item "advance paths" + remove instances corresponding to terminated paths
%    \item for each monitor repeat following steps 8.-9.
%    \item essentially just do{\textbackslash}apply the $\delta'$ from monitor instance construction
%    \item if ending up rejecting after state change $\Rightarrow$ signal violation
%\end{enumerate}
%\end{definition}
%\tbchecked{This algorithm can be generalized easily. The space consumption is in $\bigO(\card{\text{template}} + 2^\text{\# input paths})$}
%In the case of a $\hyperltl$ formula with exactly two quantifers/trace variables, detecting transitivity enables us to monitor many traces with only ever looking at two at a time. In fact it suffices to save one of the traces, let's call this $t$, and monitor any trace $t'$ by just observing $t$ and $t'$.
%\todo{Detecting symmetry would be helpful, this would reduce the number of monitor automata to ${{m+n-1} \choose n}$}

In contrast to previous approaches, our algorithm returns a witness for violation.
This highly desired property comes with a price. In constructed worst case scenarios, we have to remember every system trace in order to return an explicit witness.
However, it turns out that practical hyperproperties satisfy certain properties such that the majority of traces can be pruned during the monitoring process.

